Comprehensive Evaluation of Large Language Models for Topic Modeling

Recent work utilizes Large Language Models (LLMs) for topic modeling, generating comprehensible topic labels for given documents. However, their performance has mainly been evaluated qualitatively, and there remains room for quantitative investigation of their capabilities. In this paper, we quantitatively evaluate LLMs from multiple perspectives: the quality of topics, the impact of LLM-specific concerns, such as hallucination and shortcuts for limited documents, and LLMs' controllability of topic categories via prompts. Our findings show that LLMs can identify coherent and diverse topics with few hallucinations but may take shortcuts by focusing only on parts of documents. We also found that their controllability is limited.

==> components/figure_overview.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{components/parallel_overview.drawio.png}
        \caption{Parallel Prompting}
    \end{subfigure}
    
    \vspace{1em} % Adjust the vertical space between the subfigures
    
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=0.684\columnwidth]{components/sequential_overview.drawio.png} % Replace with the filename of your second image
        \caption{Sequential Prompting}
        \label{fig:second}
    \end{subfigure}
    
    \caption{\todo{delete }Topic modeling with LLMs by splitting a document set into subsets and prompting (a) in parallel or (b) sequentially.}
    \label{fig:overview}
\end{figure}

==> components/previous_version/table_coherence_and_diversity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
%\sisetup{detect-weight=true,detect-inline-weight=math}
\begin{table*}[t!]
\resizebox{\textwidth}{!}{%
%\begin{tabular}{lSSSSrSSSSrSSSS}
\begin{tabular}{lllllrllllrllll}
\hline
\multicolumn{1}{c}{\multirow{3}{*}{Model}} &
  \multicolumn{4}{c}{Tweet} &
  \multicolumn{1}{c}{} &
  \multicolumn{4}{c}{GoogleNewsT} &
  \multicolumn{1}{c}{} &
  \multicolumn{4}{c}{StackOverFlow} \\ \cline{2-5} \cline{7-10} \cline{12-15} 
\multicolumn{1}{c}{} &
  \multicolumn{2}{c}{$K=5$} &
  \multicolumn{2}{c}{$K=15$} &
  \multicolumn{1}{c}{} &
  \multicolumn{2}{c}{$K=5$} &
  \multicolumn{2}{c}{$K=15$} &
  \multicolumn{1}{c}{} &
  \multicolumn{2}{c}{$K=5$} &
  \multicolumn{2}{c}{$K=15$} \\
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textit{Cv}} &
  \multicolumn{1}{c}{\textit{TU}} &
  \multicolumn{1}{c}{\textit{Cv}} &
  \multicolumn{1}{c}{\textit{TU}} &
  \multicolumn{1}{c}{\textit{\textbf{}}} &
  \multicolumn{1}{c}{\textit{Cv}} &
  \multicolumn{1}{c}{\textit{TU}} &
  \multicolumn{1}{c}{\textit{Cv}} &
  \multicolumn{1}{c}{\textit{TU}} &
  \multicolumn{1}{c}{\textit{\textbf{}}} &
  \multicolumn{1}{c}{\textit{Cv}} &
  \multicolumn{1}{c}{\textit{TU}} &
  \multicolumn{1}{c}{\textit{Cv}} &
  \multicolumn{1}{c}{\textit{TU}} \\ \hline
LDA &
  0.394 &
  0.800 &
  0.401 &
  0.568 &
   &
  0.426 &
  0.984 &
  0.406 &
  0.963 &
   &
  0.320 &
  0.928 &
  0.425 &
  0.883 \\
LDA$_{\rm{Aug}}$ &
  0.445 &
  0.968 &
  0.436 &
  0.856 &
  \textbf{} &
  0.411 &
  0.984 &
  0.381 &
  0.981 &
  \textbf{} &
  0.360 &
  0.920 &
  0.508 &
  0.952 \\
TSCTM &
  0.393 &
  \bfseries 1.000 &
  0.467 &
  0.997 &
  \multicolumn{1}{l}{} &
  0.333 &
  \bfseries 1.000 &
  0.374 &
  \bfseries 1.000 &
  \multicolumn{1}{l}{} &
  0.244 &
  \bfseries 1.000 &
  0.313 &
  \bfseries 1.000 \\
TSCTM$_{\rm{Aug}}$ &
  0.355 &
  \bfseries 1.000 &
  0.433 &
  \bfseries 1.000 &
  \multicolumn{1}{l}{} &
  0.243 &
  \bfseries 1.000 &
  0.346 &
  \bfseries 1.000 &
  \multicolumn{1}{l}{} &
  0.218 &
  \bfseries 1.000 &
  0.276 &
  \bfseries 1.000 \\
BERTopic &
  0.514 &
  \bfseries 1.000 &
  0.537 &
  \bfseries 1.000 &
   &
  0.439 &
  \bfseries 1.000 &
  0.437 &
  \bfseries 1.000 &
   &
  0.459 &
  \bfseries 1.000 &
  0.485 &
  0.971 \\
BERTopic$_{\rm{Aug}}$ &
  0.535 &
  \bfseries 1.000 &
  0.526 &
  \bfseries 1.000 &
   &
  0.412 &
  \bfseries 1.000 &
  0.417 &
  \bfseries 1.000 &
   &
  0.460 &
  \bfseries 1.000 &
  0.489 &
  0.955 \\ \hline\hline
GPT-3.5$_{\rm{Smp}}$ &
  0.492 &
  0.969 &
  0.532 &
  0.888 &
   &
  0.541 &
  0.990 &
  0.517 &
  0.943 &
   &
  0.382 &
  0.937 &
  0.464 &
  0.833 \\
\bfseries GPT-3.5$_{\rm{Seq}}$ &
  0.552 &
  0.960 &
  0.515 &
  0.920 &
   &
  0.562 &
  0.984 &
  0.489 &
  0.948 &
   &
  0.441 &
  0.896 &
  0.517 &
  0.775 \\
\bfseries GPT-3.5$_{\rm{Par}}$ &
  0.476 &
  0.992 &
  0.532 &
  0.900 &
   &
  0.571 &
  0.960 &
  0.535 &
  0.913 &
   &
  0.312 &
  0.864 &
  0.496 &
  0.913 \\ \hline
GPT-4$_{\rm{Smp}}$ &
  0.553 &
  0.988 &
  \bfseries 0.580 &
  0.981 &
  \multicolumn{1}{l}{} &
  0.573 &
  0.975 &
  0.522 &
  0.967 &
  \multicolumn{1}{l}{} &
  0.445 &
  0.908 &
  0.519 &
  0.808 \\
\bfseries GPT-4$_{\rm{Seq}}$ &
  \bfseries 0.577 &
  0.992 &
  0.551 &
  0.976 &
  \multicolumn{1}{l}{} &
  0.556 &
  0.944 &
  \bfseries 0.561 &
  0.963 &
  \multicolumn{1}{l}{} &
  0.318 &
  0.744 &
  0.532 &
  0.853 \\
\bfseries GPT-4$_{\rm{Par}}$ &
  0.562 &
  \bfseries 1.000 &
  0.576 &
  0.971 &
  \multicolumn{1}{l}{} &
  \bfseries 0.618 &
  0.976 &
  0.532 &
  0.925 &
  \multicolumn{1}{l}{} &
  \bfseries 0.466 &
  0.904 &
  \bfseries 0.571 &
  0.864 \\ \hline
\end{tabular}%
}
\caption{Topic coherence (\textit{Cv}) and diversity (\textit{TU}) results under 5 and 15 topics ($K=5$ and $K=15$). MODEL$_{\rm{Aug}}$ means the performance of the model with augmentation. The maximum \textit{TU} is 1.000 when the topic words are all different. The best scores are in \textbf{bold}.}
\label{tab:Coherence-and-Diversity-for-ACL2024}
\end{table*}

==> components/previous_version/table_coverage_and_factuality.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllrllllrllll}
\hline
\multicolumn{1}{c}{\multirow{3}{*}{Model}} &
  \multicolumn{4}{c}{Tweet} &
  \multicolumn{1}{c}{} &
  \multicolumn{4}{c}{GoogleNewsT} &
  \multicolumn{1}{c}{} &
  \multicolumn{4}{c}{StackOverFlow} \\ \cline{2-5} \cline{7-10} \cline{12-15} 
\multicolumn{1}{c}{} &
  \multicolumn{2}{c}{$K=5$} &
  \multicolumn{2}{c}{$K=15$} &
  \multicolumn{1}{c}{} &
  \multicolumn{2}{c}{$K=5$} &
  \multicolumn{2}{c}{$K=15$} &
  \multicolumn{1}{c}{} &
  \multicolumn{2}{c}{$K=5$} &
  \multicolumn{2}{c}{$K=15$} \\
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textit{DC}} &
  \multicolumn{1}{c}{\textit{Fa}} &
  \multicolumn{1}{c}{\textit{DC}} &
  \multicolumn{1}{c}{\textit{Fa}} &
  \multicolumn{1}{c}{\textit{\textbf{}}} &
  \multicolumn{1}{c}{\textit{DC}} &
  \multicolumn{1}{c}{\textit{Fa}} &
  \multicolumn{1}{c}{\textit{DC}} &
  \multicolumn{1}{c}{\textit{Fa}} &
  \multicolumn{1}{c}{\textit{\textbf{}}} &
  \multicolumn{1}{c}{\textit{DC}} &
  \multicolumn{1}{c}{\textit{Fa}} &
  \multicolumn{1}{c}{\textit{DC}} &
  \multicolumn{1}{c}{\textit{Fa}} \\ \hline
LDA &
  \bfseries 0.337 &
  \bfseries 1.000 &
  0.561 &
  \bfseries 1.000 &
   &
  0.488 &
  \bfseries 1.000 &
  0.664 &
  \bfseries 1.000 &
   &
  \bfseries 0.684 &
  \bfseries 1.000 &
  \bfseries 0.842 &
  \bfseries 1.000 \\
LDA$_{\rm{Aug}}$ &
  0.307 &
  \bfseries 1.000 &
  \bfseries 0.579 &
  0.997 &
  \textbf{} &
  \bfseries 0.531 &
  \bfseries 1.000 &
  \bfseries 0.763 &
  \bfseries 1.000 &
  \textbf{} &
  0.659 &
  \bfseries 1.000 &
  0.838 &
  \bfseries 1.000 \\
TSCTM &
  0.176 &
  \bfseries 1.000 &
  0.388 &
  \bfseries 1.000 &
  \multicolumn{1}{l}{} &
  0.405 &
  \bfseries 1.000 &
  0.740 &
  \bfseries 1.000 &
  \multicolumn{1}{l}{} &
  0.141 &
  \bfseries 1.000 &
  0.480 &
  \bfseries 1.000 \\
TSCTM$_{\rm{Aug}}$ &
  0.187 &
  \bfseries 1.000 &
  0.331 &
  0.987 &
  \multicolumn{1}{l}{} &
  0.309 &
  \bfseries 1.000 &
  0.608 &
  0.979 &
  \multicolumn{1}{l}{} &
  0.419 &
  0.888 &
  0.441 &
  \bfseries 0.888 \\
BERTopic &
  0.293 &
  \bfseries 1.000 &
  0.471 &
  \bfseries 1.000 &
   &
  0.433 &
  \bfseries 1.000 &
  0.748 &
  \bfseries 1.000 &
   &
  0.656 &
  \bfseries 1.000 &
  0.796 &
  \bfseries 1.000 \\
BERTopic$_{\rm{Aug}}$ &
  0.303 &
  \bfseries 1.000 &
  0.468 &
  \bfseries 1.000 &
   &
  0.422 &
  \bfseries 1.000 &
  0.749 &
  \bfseries 1.000 &
   &
  0.637 &
  \bfseries 1.000 &
  0.795 &
  \bfseries 1.000 \\ \hline\hline
GPT-3.5$_{\rm{Smp}}$ &
  0.191 &
  0.959 &
  0.366 &
  0.967 &
   &
  0.382 &
  0.968 &
  0.569 &
  0.956 &
   &
  0.530 &
  0.980 &
  0.634 &
  0.981 \\
\bfseries GPT-3.5$_{\rm{Seq}}$ &
  0.197 &
  0.984 &
  0.335 &
  0.967 &
   &
  0.334 &
  0.975 &
  0.583 &
  0.954 &
   &
  0.479 &
  \bfseries 1.000 &
  0.689 &
  0.994 \\
\bfseries GPT-3.5$_{\rm{Par}}$ &
  0.213 &
  \bfseries 1.000 &
  0.384 &
  0.994 &
   &
  0.321 &
  0.968 &
  0.585 &
  0.952 &
   &
  0.636 &
  \bfseries 1.000 &
  0.694 &
  \bfseries 1.000 \\ \hline
GPT-4$_{\rm{Smp}}$ &
  0.220 &
  \bfseries 1.000 &
  0.395 &
  0.995 &
  \multicolumn{1}{l}{} &
  0.366 &
  \bfseries 1.000 &
  0.665 &
  0.994 &
  \multicolumn{1}{l}{} &
  0.507 &
  \bfseries 1.000 &
  0.747 &
  0.998 \\
\bfseries GPT-4$_{\rm{Seq}}$ &
  0.224 &
  0.983 &
  0.403 &
  0.994 &
  \multicolumn{1}{l}{} &
  0.373 &
  \bfseries 1.000 &
  0.660 &
  0.951 &
  \multicolumn{1}{l}{} &
  0.554 &
  0.931 &
  0.626 &
  0.883 \\
\bfseries GPT-4$_{\rm{Par}}$ &
  0.241 &
  \bfseries 1.000 &
  0.402 &
  \bfseries 1.000 &
  \multicolumn{1}{l}{} &
  0.392 &
  \bfseries 1.000 &
  0.661 &
  0.995 &
  \multicolumn{1}{l}{} &
  0.578 &
  \bfseries 1.000 &
  0.754 &
  \bfseries 1.000 \\ \hline
\end{tabular}%
}
\caption{Document coverage (\textit{DC}) and factuality (\textit{Fa}) results under 5 and 15 topics ($K=5$ and $K=15$). MODEL$_{\rm{Aug}}$ means the performance of the model with augmentation. Baseline models without data augmentation discover topics based only on documents, so that the values of factuality are 1.000 The best scores are in \textbf{bold}.}
\label{tab:Coherence-and-Diversity-for-ACL2024}
\end{table*}

==> sections/acknowledgements.tex <==
\section*{Acknowledgements}
This work was supported by JSPS KAKENHI Grant Number JP24H00809, Japan.
